Self-supervised Mamba-based Mastoidectomy Shape Prediction for Cochlear Implant Surgery

Cochlear Implant (CI) procedures require the insertion of an electrode array into the cochlea within the inner ear. To achieve this, mastoidectomy, a surgical procedure involving the removal of part of the mastoid region of the temporal bone using a high-speed drill provides safe access to the cochlea through the middle and inner ear. In this paper, we propose a novel Mamba-based method to synthesize the mastoidectomy volume using only preoperative Computed Tomography (CT) scans, where the mastoid remains intact. Our approach introduces a self-supervised learning framework designed to predict the mastoidectomy shape and reconstruct a 3D post-mastoidectomy surface directly from preoperative CT scans. This reconstruction aligns with intraoperative microscope views, enabling various downstream surgical applications. For training, we leverage postoperative CT scans to bypass manual data cleaning and labeling, even when the region removed during mastoidectomy is affected by challenges such as metal artifacts, low signal-to-noise ratio, or electrode wiring. Our method achieves a mean Dice score of 0.70 in estimating mastoidectomy regions, demonstrating its effectiveness for accurate and efficient surgical preoperative planning.

==> credit.tex <==
\begin{credits}
\subsubsection{\ackname} This work was supported in part by grants R01DC014037 and R01DC008408 from NIDCD. This work is solely the responsibility of the authors and does not necessarily reflect the views of this institute.
\end{credits}

==> equations/L_smooth.tex <==
\begin{equation}
    L_{smooth}(\delta) = \sum_{i=1}^{N}\left\| \nabla \left( \delta_{i} \right) \right\|^2
\label{Eq: smooth_loss}
\end{equation} 
In Eq. \ref{Eq: smooth_loss}, we define $\frac{\partial{\delta}}{\partial{x}} \approx \delta(i_x+1, i_y, i_z) - \delta(i_x, i_y, i_z)$, and the same rule applies to the $\frac{\partial{\delta}}{\partial{y}}$ and $\frac{\partial{\delta}}{\partial{z}}$. A lower $L_{smooth}$ value indicates higher smoothness in image volumes.

==> figures/future_work.tex <==
% \setlength{\fboxsep}{0pt}
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/future_work/6088_3d.PNG}}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/future_work/6320_3d.PNG}}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/future_work/6239_3d.PNG}}
    \end{subfigure}

    \begin{subfigure}[b]{0.3\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/future_work/6088_2d.PNG}}
         \subcaption{Case 1}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/future_work/6320_2d.PNG}}
         \subcaption{Case 2}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/future_work/6239_2d.PNG}}
         \subcaption{Case 3}
    \end{subfigure}
\caption{Feature matching between 3D meshes extracted from synthesized preoperative CTs and the corresponding 2D scenes. Similar features are circled in the same color.}
\label{fig:future_work}
\end{figure}
 % Yellow circles in (a) show partially removed but not fully removed features in 3D mesh compared to the 2D microscope view.

==> figures/network_structure_resnet.tex <==
\begin{figure}[h]
\centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,439); %set diagram left start at 0, and has height of 439

%Shape: Rectangle [id:dp6953599152793437] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (19.65,121.53) -- (236.34,121.53) -- (236.34,253.86) -- (19.65,253.86) -- cycle ;
%Shape: Rectangle [id:dp010190844981245228] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (24.29,132.2) -- (91.49,132.2) -- (91.49,205.51) -- (24.29,205.51) -- cycle ;
%Straight Lines [id:da9924459534025084] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (41.43,132.2) -- (42.12,205.51) ;
%Straight Lines [id:da9838887841977698] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (57.89,132.2) -- (58.58,205.51) ;
%Straight Lines [id:da06737033652952518] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (74.35,132.2) -- (75.03,205.51) ;
%Straight Lines [id:da8837110854119575] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (33.89,80.03) -- (34.09,128.15) ;
\draw [shift={(34.1,130.15)}, rotate = 269.76] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp3022043233712237] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (109.39,132.65) -- (159.45,132.65) -- (159.45,205.96) -- (109.39,205.96) -- cycle ;
%Straight Lines [id:da87422184950822] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (128.54,132.65) -- (129.22,205.96) ;
%Straight Lines [id:da5629480884769283] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (145.68,132.65) -- (146.37,205.96) ;
%Shape: Rectangle [id:dp9613244221705393] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (182.44,133.39) -- (232.5,133.39) -- (232.5,206.7) -- (182.44,206.7) -- cycle ;
%Straight Lines [id:da9644500337469911] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (199.58,134.39) -- (200.27,207.7) ;
%Straight Lines [id:da3780949547085487] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (216.72,134.39) -- (217.41,207.7) ;
%Straight Lines [id:da39096593661955215] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (91.78,171.44) -- (109.61,171.44) ;
\draw [shift={(109.61,171.44)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da6438783680941652] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (161.54,172.32) -- (179.37,172.32) ;
\draw [shift={(179.37,172.32)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp1601168067772636] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (266.13,135.12) -- (316.19,135.12) -- (316.19,208.42) -- (266.13,208.42) -- cycle ;
%Straight Lines [id:da8577372713696626] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (283.27,136.12) -- (283.96,209.42) ;
%Straight Lines [id:da7191376273711205] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (300.41,136.12) -- (301.1,209.42) ;
%Shape: Rectangle [id:dp604477269217071] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (340.06,135.95) -- (390.12,135.95) -- (390.12,209.26) -- (340.06,209.26) -- cycle ;
%Straight Lines [id:da6280466855968332] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (357.21,135.95) -- (357.89,209.26) ;
%Straight Lines [id:da6268662201578515] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (374.35,135.95) -- (375.04,209.26) ;
%Shape: Rectangle [id:dp7653427258347716] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (414.55,135.07) -- (464.61,135.07) -- (464.61,208.37) -- (414.55,208.37) -- cycle ;
%Straight Lines [id:da49724669394698995] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (431.69,135.07) -- (432.38,208.37) ;
%Straight Lines [id:da15493774763046397] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (448.84,135.07) -- (449.52,208.37) ;
%Straight Lines [id:da24515870944782137] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (316.64,172.18) -- (335.27,172.37) ;
\draw [shift={(337.27,172.39)}, rotate = 180.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da6713999268004597] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (390.93,171.44) -- (409.52,171.39) ;
\draw [shift={(411.52,171.39)}, rotate = 179.86] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da19663508781484773] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (455.72,86.89) -- (455.83,134.21) ;
\draw [shift={(455.72,84.89)}, rotate = 89.86] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Brace [id:dp7367278426947941] 
\draw   (46.48,216.64) .. controls (46.49,221.31) and (48.83,223.63) .. (53.5,223.62) -- (118.26,223.42) .. controls (124.93,223.4) and (128.27,225.72) .. (128.28,230.39) .. controls (128.27,225.72) and (131.59,223.38) .. (138.26,223.36)(135.26,223.37) -- (203.02,223.15) .. controls (207.69,223.14) and (210.01,220.8) .. (210,216.13) ;
%Shape: Brace [id:dp7052406851852426] 
\draw   (279.82,215.64) .. controls (279.83,220.31) and (282.17,222.63) .. (286.84,222.62) -- (351.6,222.41) .. controls (358.27,222.39) and (361.61,224.71) .. (361.63,229.38) .. controls (361.61,224.71) and (364.93,222.37) .. (371.6,222.35)(368.6,222.36) -- (436.36,222.15) .. controls (441.03,222.14) and (443.35,219.8) .. (443.34,215.13) ;
%Shape: Rectangle [id:dp5695442116660883] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (137.36,61.98) -- (370.86,61.98) -- (370.86,93.94) -- (137.36,93.94) -- cycle ;

%Straight Lines [id:da6767201393100797] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (83,131) -- (83,73) -- (134.63,72.83) ;
\draw [shift={(136.63,72.82)}, rotate = 179.81] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8227933549178987] 
\draw [color={rgb, 255:red, 139; green, 87; blue, 42 }  ,draw opacity=1 ]   (152.68,132.65) -- (152.48,96.95) ;
\draw [shift={(152.47,94.95)}, rotate = 89.68] [fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da05329054180572568] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.84 ]   (224.72,133.39) -- (224.52,97.69) ;
\draw [shift={(224.51,95.69)}, rotate = 89.68] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9293946285043458] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.84 ]   (274,133) -- (274,94) ;
\draw [shift={(274,135)}, rotate = 270] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.84 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da19647074512463014] 
\draw [color={rgb, 255:red, 139; green, 87; blue, 42 }  ,draw opacity=1 ]   (348,133) -- (348,94.25) ;
\draw [shift={(348,135)}, rotate = 270] [fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da7387614236690561] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (422,132) -- (422,77) -- (371,77) ;
\draw [shift={(422,134)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;

% Text Node
\draw (144,71) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Skip connections with convolution block}};
% Text Node
\draw (28.58,51.44) node [anchor=north west][inner sep=0.75pt]    {$\rho $};
% Text Node
\draw (242.18,168) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (449.83,59.79) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (81.65,233.7) node [anchor=north west][inner sep=0.75pt]   [align=left] {Freeze Encoder};
% Text Node
\draw (67.53,259.57) node [anchor=north west][inner sep=0.75pt]   [align=left] {Pretrained ResNet-50};
% Text Node
\draw (321.3,230.68) node [anchor=north west][inner sep=0.75pt]   [align=left] {Train Decoder};
% Text Node
\draw (26.04,186.2) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (43.68,180.06) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (59.36,188.4) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (75.87,199.26) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {MaxPool};
% Text Node
\draw (111.15,186.65) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (129.79,180.51) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (146.46,188.85) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (184.19,187.39) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (201.83,180.25) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (217.5,189.59) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (267.88,184.12) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (285.52,178.97) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (301.2,186.32) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (341.81,189.95) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (359.46,178.81) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (375.13,188.15) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (416.3,189.07) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (433.94,178.92) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (449.62,189.27) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
\end{tikzpicture}
\caption{2D UNet++ with pretrained ResNet-50 backbone.}
\label{fig:network_structure}
\end{figure}

==> figures/network_structure_resnet2.tex <==
\begin{figure}[]
\centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt 

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.75,xscale=0.75]
%uncomment if require: \path (0,462); %set diagram left start at 0, and has height of 462

%Shape: Rectangle [id:dp11306659863827828] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (92.14,87) -- (337.3,87) -- (337.3,358.5) -- (92.14,358.5) -- cycle ;
%Shape: Rectangle [id:dp01968130466878837] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (99.9,108.04) -- (175.93,108.04) -- (175.93,180.92) -- (99.9,180.92) -- cycle ;
%Straight Lines [id:da6300579937415003] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (119.3,108.04) -- (120.07,180.92) ;
%Straight Lines [id:da6203830183582361] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (137.91,108.04) -- (138.69,180.92) ;
%Straight Lines [id:da9931399221757048] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (156.53,108.04) -- (157.31,180.92) ;

%Straight Lines [id:da5098274305762373] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (110.76,57.17) -- (110.99,105) ;
\draw [shift={(111,107)}, rotate = 269.73] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp6961278581300144] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (190.45,165.49) -- (247.08,165.49) -- (247.08,238.37) -- (190.45,238.37) -- cycle ;

%Straight Lines [id:da4595255700153775] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (209.84,165.49) -- (210.62,238.37) ;
%Straight Lines [id:da2022346463535898] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (229.24,165.49) -- (230.01,238.37) ;

%Shape: Rectangle [id:dp05865047110606414] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (262.82,227.22) -- (319.46,227.22) -- (319.46,300.1) -- (262.82,300.1) -- cycle ;

%Straight Lines [id:da6991811594790975] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (282.22,227.22) -- (282.99,300.1) ;
%Straight Lines [id:da793685724310221] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (301.61,227.22) -- (302.39,300.1) ;

%Straight Lines [id:da677706731917155] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (178.26,144.05) -- (198.43,144.05) -- (198.43,162.63) ;
\draw [shift={(198.43,164.63)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da7447012022432397] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (251.18,204.93) -- (271.36,204.93) -- (271.36,223.51) ;
\draw [shift={(271.36,225.51)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp780258379524298] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (366.51,228.94) -- (423.14,228.94) -- (423.14,301.82) -- (366.51,301.82) -- cycle ;

%Straight Lines [id:da2727292208833525] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (385.9,228.94) -- (386.68,301.82) ;
%Straight Lines [id:da27239238439680835] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (405.3,228.94) -- (406.07,301.82) ;

%Shape: Rectangle [id:dp5988640149712574] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (438.16,163.77) -- (494.79,163.77) -- (494.79,236.65) -- (438.16,236.65) -- cycle ;

%Straight Lines [id:da9165089350888519] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (457.55,163.77) -- (458.33,236.65) ;
%Straight Lines [id:da817436909409273] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (476.95,163.77) -- (477.72,236.65) ;

%Shape: Rectangle [id:dp4147950389712689] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (506.43,108.9) -- (563.06,108.9) -- (563.06,181.78) -- (506.43,181.78) -- cycle ;

%Straight Lines [id:da9245615218349669] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (525.82,108.9) -- (526.6,181.78) ;
%Straight Lines [id:da5847825875376846] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (545.22,108.9) -- (545.99,181.78) ;

%Straight Lines [id:da4230636976950708] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (415.66,228.08) -- (415.66,211.79) -- (433.83,211.79) ;
\draw [shift={(435.83,211.79)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da9526060358848988] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (484.7,160.34) -- (484.7,144.05) -- (502.88,144.05) ;
\draw [shift={(504.88,144.05)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da5015307388206409] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ]   (535.01,62) -- (535.13,109.04) ;
\draw [shift={(535,60)}, rotate = 89.85] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Brace [id:dp09558454797854565] 
\draw   (116,316) .. controls (116.01,320.67) and (118.35,322.99) .. (123.02,322.98) -- (198.52,322.78) .. controls (205.19,322.77) and (208.53,325.09) .. (208.54,329.76) .. controls (208.53,325.09) and (211.85,322.75) .. (218.52,322.73)(215.52,322.74) -- (294.02,322.53) .. controls (298.69,322.52) and (301.01,320.19) .. (301,315.52) ;
%Straight Lines [id:da6580720661049216] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (185,129.5) -- (297,129.5) ;
%Straight Lines [id:da2794289232488052] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (397,130.5) -- (498,129.52) ;
\draw [shift={(500,129.5)}, rotate = 179.44] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da03445611479567401] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (253,187.5) -- (300,187.5) ;
%Straight Lines [id:da5986963209989237] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (397,187.5) -- (430,187.5) ;
\draw [shift={(432,187.5)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Brace [id:dp14595021328623192] 
\draw   (377,315) .. controls (377.01,319.67) and (379.35,321.99) .. (384.02,321.98) -- (459.52,321.78) .. controls (466.19,321.77) and (469.53,324.09) .. (469.54,328.76) .. controls (469.53,324.09) and (472.85,321.75) .. (479.52,321.73)(476.52,321.74) -- (555.02,321.53) .. controls (559.69,321.52) and (562.01,319.19) .. (562,314.52) ;
%Shape: Rectangle [id:dp15536106614173473] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (305,94.5) -- (390,94.5) -- (390,214.5) -- (305,214.5) -- cycle ;

% % Text Node for scale 1
% \draw (548,164.88) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Sigmoid};
% % Text Node
% \draw (527.14,180) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% % Text Node
% \draw (509.48,162.69) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% % Text Node
% \draw (480,219.76) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% % Text Node
% \draw (458.87,235) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% % Text Node
% \draw (441.21,217.56) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% % Text Node
% \draw (408,284.93) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% % Text Node
% \draw (387.22,300) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% % Text Node
% \draw (369.56,282.73) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% % Text Node
% \draw (305,283.21) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% % Text Node
% \draw (283.53,298) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% % Text Node
% \draw (265.88,281.01) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% % Text Node
% \draw (232,221.48) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% % Text Node
% \draw (211.16,238) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% % Text Node
% \draw (193.5,219.28) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% % Text Node
% \draw (159,174.88) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {MaxPool};
% % Text Node
% \draw (140,164.03) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% % Text Node
% \draw (120.61,180) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% % Text Node
% \draw (102.96,161.83) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% % Text Node
% \draw (316,117) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Skip }\\{\small connections }\\{\small with }\\{\small convolution }\\{\small block \cite{zhou2019unetplusplus}}};
% % Text Node
% \draw (105.54,42) node [anchor=north west][inner sep=0.75pt]    {$\rho $};
% % Text Node
% \draw (336.39,265) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% % Text Node
% \draw (529.13,42) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% % Text Node
% \draw (163.7,335) node [anchor=north west][inner sep=0.75pt]   [align=left] {Freeze Encoders};
% % Text Node
% \draw (150,368) node [anchor=north west][inner sep=0.75pt]   [align=left] {Pretrained ResNet-50};
% % Text Node
% \draw (428,333) node [anchor=north west][inner sep=0.75pt]   [align=left] {Train Decoders};

% Text Node for scale factor 0.75
\draw (544,174) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Sigmoid};
% Text Node
\draw (527.14,160) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (509.48,162.69) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (480,219.76) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (458.87,215) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (441.21,217.56) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (408,284.93) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (387.22,280) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (369.56,282.73) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (305,283.21) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (283.53,278) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (265.88,281.01) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (232,221.48) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (211.16,218) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (193.5,219.28) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (158,177) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {MaxPool};
% Text Node
\draw (140,164.03) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {ReLU};
% Text Node
\draw (120.61,160) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {BN};
% Text Node
\draw (102.96,161.83) node [anchor=north west][inner sep=0.75pt]  [rotate=-269.05] [align=left] {Conv};
% Text Node
\draw (305,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Skip }\\{\small connections }\\{\small with }\\{\small convolution }\\{\small block \cite{zhou2019unetplusplus}}};
% Text Node
\draw (105.54,42) node [anchor=north west][inner sep=0.75pt]    {$\rho $};
% Text Node
\draw (336.39,265) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (529.13,42) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (160,335) node [anchor=north west][inner sep=0.75pt]   [align=left] {Freeze Encoders};
% Text Node
\draw (140,368) node [anchor=north west][inner sep=0.75pt]   [align=left] {Pretrained ResNet-50};
% Text Node
\draw (428,333) node [anchor=north west][inner sep=0.75pt]   [align=left] {Train Decoders};

\end{tikzpicture}
\caption{UNet++ with pretrained ResNet-50 backbone, the encoders are highlighted in blue, and the decoders are highlighted in red. We freeze the encoders and train only the neural network decoders on our dataset. In the final activation layer, the sigmoid function is used to constrain the output values fall within a range between 0 and 1.}
\label{fig:network_structure} % Optional: if you want to reference the figure in your text
\end{figure}

==> figures/overview1.tex <==

\begin{figure}[h]
\centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,366); %set diagram left start at 0, and has height of 366

%Image [id:dp04985429909905015] 
\draw (133.74,120.38) node  {\fbox{\includegraphics[width=46.12pt,height=48.04pt]{figures/overview/3389_right_preop.png}}};
%Straight Lines [id:da7548488511529232] 
\draw    (171.52,124.96) -- (189.72,124.96) ;
\draw [shift={(191.72,124.96)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp5075060272043457] 
\draw   (196.02,86.61) -- (207.44,86.61) -- (207.44,159.82) -- (196.02,159.82) -- cycle ;
%Shape: Rectangle [id:dp9905265751013906] 
\draw   (251.03,86.52) -- (262.45,86.52) -- (262.45,159.73) -- (251.03,159.73) -- cycle ;
%Straight Lines [id:da7318526237001484] 
\draw    (265,125) -- (283.71,125.79) ;
\draw [shift={(285.71,125.87)}, rotate = 182.41] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Image [id:dp6245935950340661] 
\draw (323.92,124.96) node  {\fbox{\includegraphics[width=46.78pt,height=48.04pt]{figures/overview/3389_right_output.png}}};
%Straight Lines [id:da4855113236477412] 
\draw    (361.25,125.87) -- (386.48,125.87) ;
\draw [shift={(388.48,125.87)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Flowchart: Summing Junction [id:dp7860787283221131] 
\draw   (395.51,125.87) .. controls (395.51,121.57) and (398.85,118.09) .. (402.98,118.09) .. controls (407.1,118.09) and (410.44,121.57) .. (410.44,125.87) .. controls (410.44,130.17) and (407.1,133.65) .. (402.98,133.65) .. controls (398.85,133.65) and (395.51,130.17) .. (395.51,125.87) -- cycle ; \draw   (397.7,120.37) -- (408.26,131.37) ; \draw   (408.26,120.37) -- (397.7,131.37) ;
%Straight Lines [id:da03850269106034809] 
\draw    (417.47,125.87) -- (444.46,125.87) ;
\draw [shift={(446.46,125.87)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Image [id:dp569968397908204] 
\draw (482.91,124.96) node  {\fbox{\includegraphics[width=46.78pt,height=48.04pt]{figures/overview/3389_right_output2.png}}};
%Image [id:dp51617019234871] 
\draw (482.82,220.92) node  {\fbox{\includegraphics[width=46.78pt,height=48.04pt]{figures/overview/3389_right_postop.png}}};
%Straight Lines [id:da508115717215246] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (519,122) -- (554,122) -- (555,224) -- (520,224) ;
\draw [shift={(517,122)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da5476263888087551] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (328,219) -- (327.76,163.76) ;
\draw [shift={(327.75,161.76)}, rotate = 89.75] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da3067217841729828] 
\draw    (133.74,71.88) -- (133.74,49.92) -- (402.54,49) -- (401.69,104.2) ;
\draw [shift={(401.66,106.2)}, rotate = 270.88] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Shape: Rectangle [id:dp29554251195450276] 
\draw   (212.02,103) -- (221,103) -- (221,148.82) -- (212.02,148.82) -- cycle ;
%Shape: Rectangle [id:dp18357304257344298] 
\draw   (238.02,103) -- (247,103) -- (247,148.82) -- (238.02,148.82) -- cycle ;

% Text Node
\draw (222.67,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (209.92,61.53) node [anchor=north west][inner sep=0.75pt]    {$f_{\theta }( \rho )$};
% Text Node
\draw (319.24,73.43) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (129.5,73.43) node [anchor=north west][inner sep=0.75pt]    {$\rho $};
% Text Node
\draw (461.59,73.43) node [anchor=north west][inner sep=0.75pt]    {$\rho \otimes \delta $};
% Text Node
\draw (477.65,260) node [anchor=north west][inner sep=0.75pt]    {$\omega $};
% Text Node
\draw (420,165.26) node [anchor=north west][inner sep=0.75pt]    {$L_{msssim\_scc}( \omega ,\ \rho \otimes \delta )$};
% Text Node
\draw (296.9,218.97) node [anchor=north west][inner sep=0.75pt]    {$L_{smooth}( \delta )$};


\end{tikzpicture}

\caption{Framework overview. We compare predicted mastoidectomy in preoperative CT $\rho \otimes \delta$ with $\omega$ using similarity-based loss function $L_{msssim\_scc}$. A smoothing term $L_{smooth}$ is also applied to $\delta$ to further reduce noise output by network $f_{\theta}$.}
\label{fig:overview1} % Optional: if you want to reference the figure in your text
\end{figure}

==> figures/preop_postop.tex <==
% \setlength{\fboxsep}{0pt}
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.112\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/379_left_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/8409_right_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/7410_right_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/745_right_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6031_left_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6147_right_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6514_left_preop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6962_left_preop.png}}
    \end{subfigure}

    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/379_left_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/8409_right_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/7410_right_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/745_right_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6031_left_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6147_right_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6514_left_postop.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/preop_postop/6962_left_postop.png}}
    \end{subfigure}
\caption{Each column represents an individual case in our dataset. The top row shows preoperative CTs, while the bottom row displays the corresponding postoperative CTs.}
\label{fig:preop_postop}
\end{figure}

==> figures/qualitative.tex <==
\setlength{\fboxsep}{0pt}
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.112\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/799_left.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/1807_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/4862_left.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/5198_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/5671_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/5736_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/5738_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/preop/5752_left.nii.png}}
    \end{subfigure}

    \begin{subfigure}[b]{0.112\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/799_left.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/1807_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/4862_left.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/5198_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/5671_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/5736_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/5738_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/comparison/5752_left.png}}
    \end{subfigure}

    \begin{subfigure}[b]{0.112\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/799_left.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/1807_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/4862_left.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/5198_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/5671_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/5736_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/5738_right.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/output/5752_left.png}}
    \end{subfigure}

    \begin{subfigure}[b]{0.112\textwidth}
        \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/799_left.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/1807_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/4862_left.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/5198_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/5671_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/5736_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/5738_right.nii.png}}
    \end{subfigure}
    \begin{subfigure}[b]{0.112\textwidth}
         \fbox{\includegraphics[width=\textwidth]{figures/qualitative/postop/5752_left.nii.png}}
    \end{subfigure}
    
\caption{Overall performance. The first row displays preoperative CTs. In the second row, predicted mastoidectomy areas are in cyan, ground truth in yellow, and their overlap in magenta. The third row shows the synthesized mastoidectomy on preoperative CTs, while the last row presents postoperative CTs.}
\label{fig:qualitative}
\end{figure}

==> figures/quantitative.tex <==
% \setlength{\fboxsep}{0pt}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/quantitative/metrics.png}
\caption{Performance evaluation using box plots.}
\label{fig:quantitative}
\end{figure}
